DIVA: A Dirichlet Process Mixtures Based Incremental Deep Clustering Algorithm via Variational Auto-Encoder

Generative model-based deep clustering frameworks excel in classifying complex data, but are limited in handling dynamic and complex features because they require prior knowledge of the number of clusters. In this paper, we propose a nonparametric deep clustering framework that employs an infinite mixture of Gaussians as a prior. Our framework utilizes a memoized online variational inference method that enables the "birth" and "merge" moves of clusters, allowing our framework to cluster data in a "dynamic-adaptive" manner, without requiring prior knowledge of the number of features. We name the framework as DIVA, a Dirichlet Process-based Incremental deep clustering framework via Variational Auto-Encoder. Our framework, which outperforms state-of-the-art baselines, exhibits superior performance in classifying complex data with dynamically changing features, particularly in the case of incremental features. We released our source code implementation at: https://github.com/Ghiara/diva

==> outdated/08_global_rebuttal.tex <==
\clearpage
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{equation}{0}
\setcounter{page}{1}


% \begin{table}[htbp]
%   \caption{Average unsupervised clustering accuracy (\%) of Vanilla DPMM with incremental feature learning on MNIST, Fashion-MNIST and Reuters10k.}
%   \centering
%   \small
% %   \resizebox{0.9\textwidth}{!}{
%   \begin{tabular}{lcclc}
%     \toprule 
%     \# features     & MNIST     & Fashion-MNIST   & \# features     & Reuters10k     \\
%     \midrule
%     3 features    & $84.71 [\pm0.68]$ & $78.15 [\pm0.01]$ & 2 features & $64.41 [\pm0.34]$ \\
%     5 features    & $63.31 [\pm0.19]$ & $48.77 [\pm0.04]$ & 3 features & $47.08 [\pm0.23]$ \\
%     7 features    & $59.18 [\pm0.43]$ & $39.57 [\pm0.02]$ & 4 features & $48.30 [\pm0.42]$ \\
%     10 features   & $56.30 [\pm0.30]$ & $39.22 [\pm0.01]$ &  &  \\
%     \bottomrule
%   \end{tabular}
% %   }   
% \end{table}
%
\begin{table}[htbp]
  \caption{Average unsupervised clustering accuracy (\%) of state-of-the-art non-parametric baselines VSB-DPM, DDPM, vanilla DPMM compared with DIVA on MNIST, Fashion-MNIST, Reuters10k and HAR. Each trial runs with 3 times and we report their average performances.}
  \centering
  \small
%   \resizebox{0.9\textwidth}{!}{
  \begin{tabular}{lcccc}
    \toprule 
    \# features     & MNIST     & Fashion-MNIST     & Reuters10k   & HAR  \\
    \midrule
    VSB-DVM    & $78.62 [\pm0.02]$ & $63.56 [\pm0.25]$ & $69.91 [\pm1.90]$ & $63.83 [\pm0.32]$\\
    DDPM    & $88.07 [\pm1.02]$ & $70.41 [\pm1.41]$ & $69.30 [\pm0.27]$ & $73.82 [\pm0.58]$\\
    Vanilla DPMM & $56.30 [\pm0.30]$ & $39.22 [\pm0.01]$ & $48.30 [\pm0.42]$ & $65.05 [\pm0.01]$\\
    DIVA    & $\mathbf{91.02 [\pm0.18]}$ & $\mathbf{71.91 [\pm0.21]}$ & $\mathbf{82.44 [\pm1.78]}$ & $\mathbf{86.78 [\pm0.03]}$\\
    \bottomrule
  \end{tabular}
%   }   
\end{table}
%
\begin{table}[htbp]
  \caption{Clustering performance of DIVA on MNIST, Fashion-MNIST, Reuters10k, HAR, Cifar10, and Svhn. We employ metrics ``Homogeneity'', ``Adjusted Rand Index (ARI)'', and ``Normalized Mutual Information (NMI)''. We report the highest scores achieved across three trials for each metric, where higher values indicate better performance.}
  \centering
  \small
%   \resizebox{0.9\textwidth}{!}{
  \begin{tabular}{lcccccc}
    \toprule 
    Metrics     & MNIST     & Fashion-MNIST  & Reuters10k   & HAR  & Cifar10 & Svhn \\
    \midrule
    Homogeneity     & $0.741$ & $0.724$ & $0.760$ & $0.686$ & $0.893$ & $0.697$\\
    ARI             & $0.624$ & $0.579$ & $0.736$ & $0.658$ & $0.900$ & $0.547$\\
    NMI             & $0.851$ & $0.840$ & $0.864$ & $0.814$ & $0.944$ & $0.822$\\
    \bottomrule
  \end{tabular}
%   }   
\end{table}

\begin{figure}[H]
    \centering
    \resizebox{0.7\textwidth}{!}{
    \begin{subfigure}[!t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{imgs/rebuttal/cifar10_rebuild1.pdf}
        \caption{cifar cluster 1}
    \end{subfigure}
    \begin{subfigure}[!t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{imgs/rebuttal/cifar10_rebuild2.pdf}
        \caption{cifar cluster 2}
    \end{subfigure}
    \begin{subfigure}[!t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{imgs/rebuttal/cifar10_rebuild3.pdf}
        \caption{cifar cluster 3}
    \end{subfigure}
    \begin{subfigure}[!t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{imgs/rebuttal/cifar10_rebuild4.pdf}
        \caption{cifar cluster 4}
    \end{subfigure}
    }
    ~~~~~
    \centering
    \resizebox{0.7\textwidth}{!}{
    \begin{subfigure}[!t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{imgs/rebuttal/svhn_rebuild1.pdf}
        \caption{svhn cluster 1}
    \end{subfigure}
    \begin{subfigure}[!t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{imgs/rebuttal/svhn_rebuild2.pdf}
        \caption{svhn cluster 2}
    \end{subfigure}
    \begin{subfigure}[!t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{imgs/rebuttal/svhn_rebuild3.pdf}
        \caption{svhn cluster 3}
    \end{subfigure}
    \begin{subfigure}[!t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{imgs/rebuttal/svhn_rebuild4.pdf}
        \caption{svhn cluster 4}
    \end{subfigure}
    }
    \caption{Reconstruction images sampled from DIVA components on cifar10 (a)-(d) and svhn (e)-(h). Each component in DIVA can capture a reasonable main feature (e.g. the object in the images) with corresponding sub-features in the data (e.g. the image color style).}
    \label{fig:reconst_cifar10_svhn}
\end{figure}


